Conversational DevBots for Secure Programming: An Empirical Study on SKF Chatbot

Conversational agents or chatbots are widely investigated and used across different fields including healthcare, education, and marketing. Still, the development of chatbots for assisting secure coding practices is in its infancy. In this paper, we present the results of an empirical study on SKF chatbot, a software-development bot (DevBot) designed to answer queries about software security. To the best of our knowledge, SKF chatbot is one of the very few of its kind, thus a representative instance of conversational DevBots aiding secure software development. In this study, we collect and analyse empirical evidence on the effectiveness of SKF chatbot, while assessing the needs and expectations of its users (i.e., software developers). Furthermore, we explore the factors that may hinder the elaboration of more sophisticated conversational security DevBots and identify features for improving the efficiency of state-of-the-art solutions. All in all, our findings provide valuable insights pointing towards the design of more context-aware and personalized conversational DevBots for security engineering.

==> SKF chatbot study/sections/approach.tex <==
\section{\textbf{Background: SKF Chatbot}}
\label{sec:approach}

SKF chatbot \cite{cite5} was selected to study the relevance and effectiveness of conversational DevBots in secure software development. SKF chatbot is developed as a part of the Secure Knowledge Framework project\footnote{https://www.securityknowledgeframework.org/}. 
%\subsection{\textbf{Security Knowledge framework (SKF)}}
The OWASP\footnote{https://owasp.org/} Security Knowledge Framework (SKF) is a tool to guide developers to ensure security in all stages of software development. It uses OWASP Application Security Verification Standard\cite{cite7} to educate programmers about software security vulnerabilities and how to prevent them. 

%SKF is available as an open source web application. SKF maintains a huge knowledge base of information related to different software security vulnerabilities. In addition to this, it tries to achieve secure development by providing security checklists for software projects. These checklists are derived from OWASP Application Security Verification Standard (ASVS) and Mobile Application Security Verification Standard (MASVS)\cite{cite6}. 


% \subsection{\textbf{SKF Chatbot}}
SKF chatbot was developed by Jain et al. \footnote{https://github.com/Priya997/SKF-Chatbot} as an extension of the SKF project to enable the users to quickly access the required information on security vulnerabilities from the knowledge bases managed by SKF. Users can ask questions about various software vulnerabilities in natural language to the bot. The chatbot mainly attempts to answer 3 types of questions about these vulnerabilities: i) Description: The chatbot gives a detailed description in natural language for the given vulnerability ii) Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability iii) Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby.

%\begin{itemize}
%    \item Description: The chatbot gives a detailed description in natural language for the given vulnerability.
%    \item Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability.
%    \item Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby. 
%\end{itemize}

\paragraph{\textbf{SKF Knowledge Base}}
The SKF knowledge base consists of information about thousands of software security vulnerabilities and their code examples. One of the main sources for the data in this knowledge base is the CWE (Common Weakness Enumeration) \cite{cite11} list. In addition to the vulnerabilities in this list, SKF maintains and updates their own list of vulnerabilities. The knowledge base data can be found in their Github repository\footnote{https://github.com/blabla1337/skf-flask/tree/main/skf/markdown/knowled- ge\_base}.
\paragraph{\textbf{Working of SKF Chatbot}}

The working of SKF chatbot can be divided into 3 main steps: \textit{Intent Classification, Entity Recognition and Response Generation}

Intent Classification: First step in answering a natural language question from a user is to identify the intent behind the question. SKF chatbot uses a prominent Natural Language Processing (NLP) algorithm called Multinomial Naive Bayes (MNB) classifier to predict the intent of a question. MNB classifier is a frequently employed algorithm to classify textual data. Based on the predictions from this probabilistic learning algorithm, the chatbot decides if the user is asking for the description, solution or a code example for the vulnerability.

Entity Recognition: In this step, the chatbot tries to understand the vulnerability for which the user is requesting information. This is done by separating the keywords from the common words in the question. SKF chatbot achieves this with the help of a domain independent keyword extraction algorithm called Rapid Automatic Keyword Extraction (RAKE) \cite{cite10}.

Response Generation: Depending on the intent and the entity extracted from the question, the bot generates a response by parsing the knowledge base.

\paragraph{\textbf{SKF Chatbot Deployment}}
SKF allows 2 ways to deploy and use the chatbot: Gitter\footnote{https://gitter.im/} and Terminal. Gitter is an open source instant messaging platform for software developers and Github users. The Gitter version of the chatbot allows users to chat with the bot in a chat room on Gitter platform. Alternatively, the terminal version allows the users to run the chatbot on their local machines via terminal. The terminal version of the chatbot was used in our study. A depiction of the chatbot answering questions in the terminal version is shown in Figure \ref{fig:chatbot}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=.2]{figures/skf.jpeg}
    \caption{Terminal version of SKF chatbot}
    \label{fig:chatbot}
\end{figure}

==> SKF chatbot study/sections/conclusion.tex <==
\section{\textbf{Conclusions and Future Work}}
\label{sec:conclusion}

%This paper investigates how well a conversational security DevBot can assist developers in removing security vulnerabilities in a software application. We conducted an empirical study which required the participants to remove 2 security vulnerabilities in a Java web application with and without using a state of the art conversational agent for software security called SKF chatbot. We collected the feedback from the participants to understand the benefits and limitations of using SKF chatbot and by extension conversational security DevBots in general. Our findings show that there is room for improvement in chatbots for secure programming. 
%Even though there are significant advancements in technology for creating efficient conversational agents in multiple areas, the field of secure software development is lagging behind. 

Supporting developers in their programming practices is of utmost importance for the generation of secure software solutions. Recent advances in AI have contributed to the emergence of DevBots aiding security-related tasks. Still, conversational approaches are in their infancy and thus demand further research and scientific insights. In this work, we have shed some light on the limitations and challenges in the development of conversational DevBots for security engineering. Overall, our findings suggest that these technologies are seen as a reliable source of security knowledge. However, they should incorporate features such as context-aware recommendations and automatic code analysis to increase their levels of user acceptance. Particularly, users would largely benefit from a conversational DevBot capable of providing context-specific answers and code examples that can be easily integrated into existing software projects.

%Answering \textbf{\textit{RQ3}}, from the study we observe that more users would prefer to use conversational DevBots for secure software development if the bots are equipped with better conversational capabilities, UI and context-aware solutions or enable follow up questions in addition to the existing features in SKF chatbot.

A security DevBot of such characteristics would require an extensive Knowledge Base (KB) comprising data on software security vulnerabilities, mitigation methods, code examples, and library dependencies, among others. Nonetheless, curating such a KB by hand can be a tedious task to carry out. Moreover, technical solutions leveraging manually-curated KBs (e.g., CogniCryptGen \cite{cite22}) cover just a small number of security use cases. Alternatively, it could be feasible to elaborate richer KBs by leveraging data from open-source projects available online. GitHub Copilot \cite{cite37} is a commercial tool that employs this approach. However, a recent study shows that 40\% of the code generated by GitHub Copilot may contain security vulnerabilities \cite{cite37}. In the future, we will investigate alternative strategies for constructing KBs suitable for conversational security DevBots, and thereby overcome some of the limitations and challenges presented in this paper. Recently, \citet{fischer2019stack} released a large dataset consisting of security labelled data-code examples extracted from Stack Overflow\footnote{https://stackoverflow.com/}. In future publications we will assess whether such a dataset can be leveraged for expanding the knowledge of security DevBot solutions.

%For future work, we plan to explore alternative ways to overcome the impediments in the creation of a knowledge base which can be used  to create a conversational security DevBot with the features identified in this paper.

%We speculate that the main reason for this is the limitation in creating an extensive knowledge base. To achieve this, the DevBot should have a knowledge base that contains extensive data on software security vulnerabilities, mitigation methods, code examples for the vulnerability and the solution, library dependencies, correct API usages etc.This knowledge can be either created manually or by crawling multiple sources on the internet. However, to create such an extensive knowledge base manually, that covers a multitude of vulnerabilities and use cases, can be tedious. A secure code generating tool called CogniCryptGen \cite{cite22} adopts the method of manually curating the knowledge base by writing security and code integration rules with the help of cryptography experts. The obvious disadvantage of the tool is that it only covers a very limited number of security use cases. The second alternative to create an extensive knowledge base is to collect data from the open source projects by crawling the internet. GitHub Copilot is a commercial tool that employs this approach to create a knowledge base. However, a recent study on GitHub Copilot shows that 40\% of the code generated for various security scenarios by the tool consists of some kind of security vulnerabilities \cite{cite37}.







==> SKF chatbot study/sections/discussion.tex <==
\section{\textbf{Discussion}} \label{sec:discussion}

In this section we discuss the results presented in Section~\ref{sec:results} to elaborate on the RQs of our study. This includes aspects related to the performance of SKF chatbot as well as envisaged features for improving chat-based security DevBots. The limitations of our experimental approach are also addressed by the end of this section.

\subsection{Performance (RQ1, RQ2, and RQ3)}

In terms of \textbf{effectiveness} (\textbf{RQ1}), self-conducted Internet searches seem to outperform the DevBot when it comes to full fixes (i.e., 7/15 against 3/15). Moreover, if we consider full and partial fixes as a whole, the SKF chatbot is still outperformed by the use of the Internet (9/15 against 11/15). 
%Hence, a considerable number of participants were not able to solve the tasks using the DevBot. 
After further inspecting the participants' answers and having a follow-up interview with some of them, we identified some drawbacks in the current DevBot approach. Particularly, participants mentioned that SKF chatbot only reacts to specific input, and performs poorly when asked follow-up questions. Such was the case of Participant 12 (P12) who said:

\begin{quote}
    \textit{P12: to me the bot was not really useful, because I asked different questions and got always the same answer}
\end{quote}

Moreover, one participant mentioned it did not provide any information on the external libraries necessary to implement the prescribed fixes. This last point is manifested in the larger number of partial fixes compared to full fixes. Despite of this limitation, some participants considered the DevBot as a good starting point when solving security vulnerabilities. For instance, P4 reported: 

\begin{quote}
    \textit{P4: For someone who was a beginner at such tasks, I needed more examples with explanation. But it was a good point to start. From the points given by the chatbot I understood what exactly I need to search. }
\end{quote}

%It could be unwise to create a chatbot that browses the internet for code examples because according to a study conducted by Nadi et al. 80 - 90\% of the cryptography API usages in open source projects are incorrect \cite{cite24}. Correctly using cryptography APIs is imperative to avoid or remove software vulnerabilities. 
%An alternative way a conversational security DevBot could help in such cases is to allow follow up questions. Follow up questions could enable the developers to clarify the solutions or the examples provided by the chatbot. 

When it comes to \textbf{usefulness} (\textbf{RQ2}), most of the participants agreed that SKF chatbot helped them to understand the nature of the vulnerabilities better than the sources they found on the Internet (Section~\ref{sec:usefulness}). In part, this could be because the DevBot reduces the time developers spend retrieving information as it provides a full description of security vulnerabilities, suitable mitigation actions, and code examples. Moreover, unlike code snippets that can be found on the Internet, the ones provided by the chatbot are seen as trustworthy and hence free of additional security vulnerabilities:

\begin{quote}
    \textit{P9: I was looking into other resources to look for specific Java code examples, i.e. API calls. So for me, it was accompanying material, as the chatbot helped me to nail down the problem itself and give me trustworthy information.}
\end{quote}

As mentioned in Section~\ref{sec:qacoverage}, 10 out of 15 participants said that the DevBot answered all their questions. However, some limitations in the Natural Language Processing (NLP) features of the bot were spotted by some of them:

\begin{quote}
    \textit{P9: My question had to match the given question exactly. I ended up with asking for very broad topics and then selecting from the given list of options to find exactly what I was looking for.}
\end{quote}

This issue may be associated with the fact that SKF chatbot uses a multinomial naive Bayes algorithm to predict the intent behind the queries. Nowadays there are much more sophisticated and versatile NLP frameworks that can be used for this purpose, and hence to improve the conversational capabilities of security DevBots. For instance, BERT \cite{cite20} is a novel language representation model which has shown promising results in question-answering and language interface applications. Another suitable approach is the so called Generative Pre-trained Transformer - 3 (GPT-3) \cite{cite21} which uses deep learning to produce human-like text. Such NLP frameworks combined with a larger knowledge base can help shaping more advanced and efficient conversational security DevBots.

%\subsection{\textbf{Developer Preferences: Chatbot or No Chatbot for Secure Programming?}}

%Adoption Intentions
%Adoption and Acceptance
%Acceptance of Security DevOps


As shown in Section~\ref{sec:usefulness}, 6 out of 8 participants were inclined towards a DevBot-aided approach for addressing future security vulnerabilities. Such \textbf{intentions} (\textbf{RQ3}) can be associated with the clarity with which information is presented by the DevBot along with its reliability, accessibility, and promptness: 

\begin{quote}
\textit{P11: The answers (of the DevBot) matched precisely the given problems. In addition the answers were correct, while answers on the Internet are sometimes incoherent and misleading. In a way the Chatbot was a trusted resource, but for explicit code examples I would nevertheless search the internet. } 
\end{quote}

Nonetheless, the DevBot adoption can be hindered due to conversational limitations (as mentioned earlier) and an unpleasant user interface (P11). Even though participants did not make explicit reference to a lack of adaptability to project-specific scenarios, it can also lessen the DevBot's usability to a large extent. 


%As discussed in the previous section, the conversational restrictions of chatbots can be remedied by using more sophisticated natural language representation models. The limitation in the user interface is very specific to SKF chatbot which can also be easily improved. The challenging problem in a security DevBot is to provide customised or context-aware solutions for software projects. To achieve this, the knowledge base of the bot needs to be fused with data on different security libraries and their correct usages. To answer the question on how to do this is currently out of the scope of this paper.

%Answering \textbf{\textit{RQ3}}, from the study we observe that more users would prefer to use conversational DevBots for secure software development if the bots are equipped with better conversational capabilities, UI and context-aware solutions or enable follow up questions in addition to the existing features in SKF chatbot.

\subsection{\textbf{Envisaged Features (RQ4)}}

Participants also gave their feedback about which \textbf{additional functionalities} (\textbf{RQ4}) would be beneficial for a conversational DevBot addressing security flaws in software projects. Besides from improvements in the UI and conversational features of the bot, they suggested adding security indicators to the prescribed solutions:

\begin{quote}
\textit{P8: Maybe give recommendations like: this solution helps in 90\% of all cases.}\\[1ex]
\textit{P11: Maybe giving it some code lines and an estimation of how secure it is? Perhaps even suggesting possible vulnerabilities.}
\end{quote}

%Besides from an improved UI and conversational skills, an additional feature suggested by the participants of the study is to add a security level indicator to the solutions provided by the bot.

Sorting and displaying the DevBots' prescriptive solutions according to their security level could improve their navigability, and hence ease their selection. Thereby, developers would become aware of the drawbacks/limitations a particular solution may entail (if any). Supporting examples in other programming languages such as Django and Ruby was another feature pointed by one of the participants (P14). A greater support for integrating solutions into specific code projects was also highlighted as a missing functionality of the DevBot (P12). 

%Sorting the prescriptive solutions in descending order of security or showing the level of security offered by different solutions can assist the developers to be aware of the security risks of the solution and make an informed choice. Option to use different programming languages for code examples is another feature preferred by the users to have in the bot. The bot should also assist the developers in integrating the solution into their projects. 

%A limitation of this study is that, the participants were given information on where the vulnerability is in the code and what the vulnerability is called.  The participants merely had to look up these vulnerabilities online or via SKF chatbot to remove it from the source code. However, in reality the developers will not be having this information when they create a software application. 

Because of our experimental approach, participants did not need to spot the vulnerabilities themselves inside the provided code snippets. Instead, vulnerabilities were given as input so they could conduct the fixes in a controlled experimental fashion. Nevertheless, supporting the detection and identification of security vulnerabilities in software projects should be a key feature of DevBot solutions. Moreover, according to \citet{cite1}, an ``ideal DevBot'' is defined as:

\begin{quote}
    \textit{... an artificial software developer which
is autonomous, adaptive, and has technical as well as social
competence.}
\end{quote}

Hence, conversational security DevBots should also be capable of mimicking the social and technical skills of software developers to create a smooth interaction with their users. 

In a nutshell, our findings suggest that conversational DevBots for software security should incorporate the following envisaged features to their design:

\begin{enumerate}
    \item Strong integration with the development environment.
    \item Automatic code analysis.
    \item Automatic vulnerability detection.
    \item Enhanced natural language interaction.
    \item Context-aware recommendations.
    \item Automatic code repair.
\end{enumerate}

Many of these features require extensive research efforts and interdisciplinary work. Current advances in machine learning, human-computer interaction, and natural language processing can certainly support this quest. Still, a stronger synergy across these disciplines will be necessary to successfully integrate their individual findings into the design of conversational DevBots for security engineering.

%Combining our findings from the study with the above definition, we believe that a conversational Security DevBot should, i)be integrated into the software project, ii) automatically analyse the code written by the developer, iii) get activated when it detects a misuse of the code or security vulnerabilities, iv) interact with the developer about the risks via natural language conversations, v) offer alternative solutions which are context-aware and sources to fix the problem and finally vi) fix the code in the project, if allowed by the user. 

%\begin{itemize}
%    \item integrated into the software project, 
    
%    \item automatically analyse the code written by the developer 
    
%    \item get activated when it detects a misuse of the code or security vulnerabilities
    
%    \item interact with the developer about the risks via natural language conversations
    
%    \item offer alternative solutions and sources to fix the problem
    
%    \item fix the code in the project, if allowed by the user 
    
%\end{itemize}

%To summarize, a conversational DevBot for software security should enable peer programming where the peer is an artificially intelligent conversational agent who is knowledgeable in secure programming. 

\subsection{Limitations}

Although this study has yielded interesting results, there are certain limitations that should be acknowledged. First of all, the size of the sample is relatively small (15) and hence the results may not be generalizable to a larger population. We could also not thoroughly investigate the existence of potential relations between the variables involved in the study (e.g: knowledge level of the users) and the perceived usefulness due to the small sample. Moreover, the study subjects were mostly students (with programming experience) which could also hinder the validity of our findings. Nevertheless, the use of students as participants remains a valid and effective approach for recreating real software engineering settings in laboratory contexts \cite{falessi2018empirical}. Therefore, we have analysed and interpreted the results of our study taking into consideration the limitations given by the sample composition and size.

Another limitation point is related to the survey instruments employed throughout the study. Particularly, some of the questions included in the survey forms may not fully capture the aspects they intended to. For instance, capturing participants' perceived usefulness may require scales containing several survey items. Hence, the outcome of this study should be seen as a first attempt in assessing the performance of conversational security DevBots, and not as ultimate conclusions. In the future we plan to extend our analysis by the means of validated scales and constructs like Technology Acceptance Model \cite{davis1985}, in order to improve the value of our results.





==> SKF chatbot study/sections/extras.tex <==

%--DONE: One of the main reasons is the ease with which one can retrieve information from the chatbot. A serious problem developers face while browsing the internet for answers is the overwhelming amount of information. The enormous number of sources on the internet makes it sometimes difficult to retrieve the relevant information. SKF chatbot helps in significantly reducing the information retrieval time and effort. SKF chatbot provides the description of the vulnerability, explains the mitigation methods and gives code examples for the defense methods which makes it extremely convenient for the developers to use it. The chatbot also allows the users to choose the programming language for the code example they request. Another advantage of SKF chatbot identified by few participants is its reliability. Even though you can find a large amount of information on the internet, it is often hard to decide the reliability and correctness of these information. SKF chatbot is specially designed to address software security related issues. Hence it can be considered as a more trusted source of information for software security. One participant pointed out the clarity and understandability of the answers given by the chatbot as a contributing factor in choosing the SKF chatbot for the removal of vulnerabilities. Some participants also appreciated the interactive nature of the chatbot. 

%--DONE: Despite getting satisfactory answers from the bot, many of the participants were not able to solve the task using SKF chatbot while using other information resources proved to give better results. After further inspection of the unanswered questions from the participants who did not get completely satisfactory answers, we found some  limitations of the bot. One of the major drawbacks identified by the participants was that the bot only responds to specific questions. 

%--DONE: The three main responses one can obtain from SKF chatbot are the description of the vulnerability, mitigation methods and code example for these mitigation methods. It is natural for the users to have follow up questions after looking at the answers given by the bot. However, the chatbot grants no provision to ask such questions. More accurately, there are indeed provisions to ask follow up questions, but the chatbot merely responds with either the same answers or fails to answer all together. Another participant mentioned that the chatbot did not have information on the external libraries used to implement a solution.  One participant pointed out the lack of domain knowledge of the chatbot. The information provided by the chatbot on the vulnerabilities were found insufficient to fully comprehend and fix the vulnerabilities.

%--DONE: To clarify the disparity in this data, a follow up interview was conducted with the 5 participants to explain their decisions. Few of the responses are given below.

%--DONE: \begin{quote}
%    \textit{P4: For someone who was a beginner at such tasks, I needed more examples with explanation. But it was a good point to start. From the points given by the chatbot I understood what exactly I need to search. }
%\end{quote}

%--DONE: \begin{quote}
%    \textit{P9: I was looking into other resources to look for specific Java code examples, i.e. API calls. So for me, it was accompanying material, as the chatbot helped me to nail down the problem itself and give me “trustworthy” information.}
%\end{quote}

%--DONE: From the above responses, we observed that the contrasting feedbacks are caused by how different participants perceive the chatbot. While some of them see the chatbot as a starting point for their search for answers, the others see it as the sole source of information to perform a task.

%\subsection{Overall Acceptance}

%Quotes from a few participants are given below regarding the versatility of the chatbot.

%---DONE:\begin{quote}
%    \textit{P9: " My question had to match the given question exactly. I ended up with asking for very broad topics and then selecting from the given list of options to find exactly what I was looking for. "}
%\end{quote}
%\begin{quote}
%    \textit{P12: " to me the bot was not really useful, because i asked different questions and got always the same answer, .. "  }
%\end{quote}

%--DONE: If the participants are choosing to not use a conversational agent that is specially designed to make their life easier then definitely the agent is missing some important features. To understand this we asked the participants about the features and characteristics they expect in such a conversational agent. Some participants mentioned that they would prefer to have a better user interface for a chatbot. The messages from the chatbot especially those that involve a large amount of text should be well formatted to make it more readable. One additional feature suggested by few of the participants is an indication of the security level of the solutions. 

%--DONE: Security vulnerabilities in software applications can be solved in multiple ways. Developers often find it hard to decide which solution to implement for their use case. It would be helpful if the chatbot can indicate how secure a given solution is. 

%--DONE: Most participants expect chatbots to have much more domain knowledge instead of limiting the questions just to description, mitigation and code examples. Expanding the code examples to more programming languages will also be a good addition to the chatbot. A few participants found it difficult to integrate the code examples for the solutions given by the chatbot into their own project. They pointed out that it would be very useful if the chatbot provided assistance in doing this. 

==> SKF chatbot study/sections/introduction.tex <==
\section{\textbf{Introduction}}
\label{sec:intro}




%%The world entered the Information Age in the mid-twentieth century. Today, anyone can have access to infinite amount of information on a variety of topics. One could go on the internet and look up how to design a rocket and find satisfying answers. 

%%Under these circumstance one would assume that it is relatively easy to develop secure software applications because of all the available resources guiding to do the same. However, the statistics from NVD (National Vulnerability Database) proves otherwise. According to NVD, over 18,000 software vulnerabilities were recorded in the year 2020. For the year 2021, the number recorded is 16,973 and counting. Despite having an extensive amount of information available online on secure practices in software development, there is a gap in the implementation of these practices in the real world projects by the developers.



%% Secure programming - importance - bots or tools to assist secure software development - chatbots - fields that use chatbots - not many chatbots in secure programming - security vulnerabilities due to code level problems - security vulnerabilities in softwares due to poor decisions made by developers - developers sacrifice security for various reasons - code scanning tools show where the error is - but no way to mitigate - how a chatbot can help - guide the developer decisions - 

Every year hundreds of organizations and companies around the world are negatively affected by severe data breaches and cyber attacks. To a large extent, this is due to a lack of adequate security measures and controls within information systems. Still, secure coding practices in software projects are far from being the norm as developers often lack of proper training, and security is more of an afterthought than an actual priority \cite{rindell2019managing}. In turn, a large number of threats and vulnerabilities emerge as a result of unsavvy decisions and poor security design practices \cite{cite26}. 

Recent advances in Artificial Intelligence (AI) in general and machine learning in particular have fostered the emergence of chatbots assisting people's decisions in different fronts and domains (e.g., healthcare, education, and marketing) \cite{adamopoulou2020overview}. Certainly, the software industry has not been the exception to chatbot applications, where conversational agents have also being proposed to support core software engineering tasks (e.g., testing and requirements analysis) \cite{cite36}. Moreover, such `DevBots' are slowly becoming popular as well in the field of cyber-security, helping developers to spot security flaws in their~code. 

Several DevBots have been proposed within the current literature to help in the identification of security flaws during development \cite{cite28,cite35,cite36}. These solutions often employ static or dynamic code analysis features for spotting and warning developers about security vulnerabilities. Still, most of these tools do not yet provide \textit{conversational support} to help fixing nor mitigating the bugs they identify \cite{cite30}. Hence, there is a call for more supportive DevBot solutions that could provide instructional content on how to improve the security of software projects through adequate coding practices.

In this work, we aim to delve into the extent to which current conversational DevBot applications assist the development of secure software systems. For this, we conducted an empirical study on SKF chatbot (SKF stands for Security Knowledge Framework), a conversational agent designed to address developers' security-related questions. Particularly, we aimed at evaluating the extent to which the assistance of SKF chatbot is deemed adequate and useful by its users. To gain insights on these performance aspects we ran a study with 15 participants in which they had to use SKF for removing code vulnerabilities. Overall, the research questions (RQs) addressed in this work are the following:

\textbf{\textit{RQ1}: How effective are conversational DevBots for secure programming?} To answer this RQ we analysed the extent to which the DevBot helped participants to remove security vulnerabilities. That is, whether it led to full, partial, or no vulnerability fixes, and compared it against the outcome when no DevBot support was provided.

%\textbf{\textit{RQ1}: How useful are conversational DevBots for secure programming?} To answer this RQ we developed a questionnaire for capturing the extent to which participants understood the nature of the vulnerabilities they had to fix, and whether they managed to find the right fix for such vulnerabilities.

%\textbf{\textit{RQ2}: How useful are conversational DevBots for secure programming?} This RQ was addressed by analysing the amount of time participants took for solving the vulnerability-fix task. That is, with and without the help of SKF chatbot. We also assessed whether the DevBot managed to answer all the questions posited by the participants along with the perceived usefulness of the tool.

\textbf{\textit{RQ2}: How useful are conversational DevBots for secure programming?} In this case we developed a questionnaire for capturing the extent to which participants understood the nature of the vulnerabilities they had to fix, and whether they managed to find the right fix for such vulnerabilities. We also assessed whether the DevBot managed to answer all of their questions along with the perceived usefulness of the tool.

\textbf{\textit{RQ3}: Do developers prefer to use a conversational DevBot when conducting security-related tasks?} To answer this RQ we included some questionnaire items assessing developers' intentions towards a DevBot-aided approach over other problem-solving strategies (e.g., a manual online search).

\textbf{\textit{RQ4}: What features do developers expect from a conversational DevBot for secure programming?} This RQ aims to identify features that could improve the effectiveness of current conversational security DevBots. For this we included some open-ended questions by the end of our study to elicit the functionalities of an ``ideal'' chatbot solution.


%Through this research questions we hope to shed some light into the missing features in existing conversational DevBots for secure programming.

%To answer the above questions, we performed a study on 15 participants using SKF chatbot for removing code-level vulnerabilities. 

Our findings suggest that there is still room for improvement in security DevBots, specially when it comes to creating an extensive knowledge base containing reliable information about (i) security vulnerabilities, (ii) fixes, (iii) correct security API usages, and (iv) correct code integration rules. Furthermore, there is a need for more context-aware solutions capable to (i) provide feedback aligned with the individual characteristics of software projects, and (ii) give personalized assistance and support to the end users.

%... and that the main reason behind this is the complexity in creating an extensive knowledge base that contains reliable information on security vulnerabilities, fixes, correct security API usages and rules on code integration. 


The remaining of this paper is organizes as follows: Section~\ref{sec:rw} gives a brief overview of the existing conversational and security DevBots as well as some background on SKF chatbot, Section~\ref{sec:methodology}
describes our research methodology, the results and their discussion is done in Sections~\ref{sec:results} and \ref{sec:discussion} respectively. We finally conclude the paper and discuss future research directions in Section~\ref{sec:conclusion}.
%%Try to include points in \cite{cite8} into the motivation and relevance of this research.

%%Contribution:

%%- Studying how existing conversational DevBots assist developers in secure programming
%% - What all developers expect from conversational DevBots for secure programming.

==> SKF chatbot study/sections/relatedWork.tex <==
\section{\textbf{Background and Related Work}}
\label{sec:rw}
%We performed a detailed literature survey on conversational bots for software development or conversational DevBots for short to understand the key characteristics that set them apart from ordinary software development tools. These characteristics were then used to analyse the existing automated tools for secure software development. Our findings helped us in choosing SKF chatbot for this empirical study.




In this section we give an overview of the current state-of-the-art in  DevBots development. We also introduce the theoretical foundations for our study, namely SKF chatbot and its main characteristics.

\subsection{Conversational and Security DevBots}

In the recent years, bots and their applications have caught the attention of researchers across different software-related disciplines \cite{cite36}. Specially, there is an increasing interest towards conversational solutions capable of interacting via natural language commands. MSRBot \cite{cite2} for instance is a conversational DevBot supporting tasks related to the mining of software repositories that can address project-specific questions like \textit{``who modified <file\_name>?''} or \textit{``what commits were submitted on <date>?''}. APIBot \cite{cite18} is another conversational agent capable of answering questions about the adequate usage of APIs, thus releasing developers from the burden of scrutinizing multiple pages of API documentation. DevBots incorporating voice-recognition features can also be found within the current literature. Such is the case of Devy \cite{cite16}, a voice-activated assistant helping software practitioners to perform high-level workflow tasks (e.g., submitting code changes for review). Still, research on voice-controlled DevBots is at a very early stage when compared to chat-based support \cite{cite36}.

Security engineering has not been the exception to DevBots and its applications. Particularly, bug identification, automated testing, and code repair are some of the tasks supported by current security DevBots \cite{cite36}. For instance, \citet{wyrich2019towards} proposed a refactoring DevBot capable of spotting code smells and fixing simple warnings. Besides, the bot can also send refactored changes to the developers in the form of pull requests. SAW-BOT \cite{serban2021saw} is another bot helping developers addressing warnings in their code. Like \cite{wyrich2019towards}, SAW-BOT generates fixes that are later suggested to developers via pull requests. Other security DevBots like Repairnator \cite{cite3} have been shaped to support code repair tasks and to monitor test failures in continuous integration. Bots detecting risky commits in open-source projects are also matter of ongoing research efforts~ \cite{cite36}.

%---NO: Software repository management for instance is a field in which DevBots have been often proposed to automate recurring tasks. Such is the case of MSRBot \cite{cite2}, capable of supporting developers in the mining of software repositories by parsing natural language queries. Source code refactoring is another recurrent (and tedious) activity that DevBots can also take over. 


%Chatbots are natural language interfaces that interact with their users to provide assistance in accessing data and services.
%There is a rising interest in chatbots in  online platforms offering different kinds of services.  

%Based on the findings of a study conducted by Brandtzaeg et al. \cite{cite8}, one of the main motivation behind using chatbots is the ease and convenience with which one can access relevant information. 

%Despite the growing advancements in chatbot technology there are only limited number of chatbots that assist in software development. 
%APIBot \cite{cite18} developed by Tian et al. is a conversational bot that takes API documentations as input and answers questions regarding API usage.
%MSRBot \cite{cite2} is another chatbot that enables the developers to extract information on their software repositories using natural language queries. 
%Xu et al. presented AnswerBot \cite{cite19} that can summarize answers from multiple posts on Stack Overflow for a given user query. In \cite{cite15}, Gottipati et al. developed a semantic search engine framework that looks for relevant answers in software threads to user queries. A voice command activated bot called Devy \cite{cite16}, is a Conversational Developer Assistant (CDA) that assists the developers in performing high-level work-flow tasks such a submitting code changes for review. Another conversational bot called TaskNavigator \cite{cite17}, answers developer queries by extracting development tasks from documentations. %Bansal et al. \cite{cite37} presented a Neural QA model trained on source code and documentation to answer subroutine questions from the developers.



%\subsection{\textbf{Conversational DevBots for Secure Programming}}
%To the extent of our knowledge, there are currently no conversational DevBots other than SKF chatbot which are specially dedicated to assist in software security related issues. However one can probably extent or modify the existing DevBots to incorporate software security applications. For instance, APIBot mentioned in the previous section, uses API documentation to answer user queries. Theoretically, it should be possible for APIBot to answer cryptography related questions if it is provided with a cryptography API documentations. 

\subsection{SKF Chatbot}

%\section{\textbf{Background: SKF Chatbot}}
%\label{sec:approach}

Unlike in other software engineering domains, conversational Dev-Bots seem to be underrepresented in the security field. Overall, very few chat-based solutions can be spotted within the current literature,  SKF chatbot\footnote{https://github.com/Priya997/SKF-Chatbot} being one among the most salient ones. SKF was developed as part of OWASP's Secure Knowledge Framework project\footnote{https://www.securityknowledgeframework.org/} to enable quick access to information on security vulnerabilities. It contains a knowledge base of common security weaknesses and vulnerabilities along with a set of code examples. Basically SKF can react to 3 type of inquiries on a particular vulnerability, namely (i) \textit{description}, (ii) \textit{solution}, and (iii) \textit{code snippet}. While the first two provide detailed information in natural language about the vulnerability and its prospective solution, the third one corresponds to a code example either in Django, Java, PHP, Flask or Ruby.

%Through SKF users can ask questions about software vulnerabilities using natural language instructions. The chatbot mainly attempts to answer 3 types of questions about these vulnerabilities: i) Description: The chatbot gives a detailed description in natural language for the given vulnerability ii) Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability iii) Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby.

%---Optional: Although SKF maintains and updates its own list of vulnerabilities, many of the entries inside its knowledge base correspond to information available in the Common Weakness Enumeration (CWE) database.

%SKF chatbot\footnote{https://github.com/Priya997/SKF-Chatbot} was selected to study the relevance and effectiveness of conversational DevBots in secure software development. SKF chatbot is developed as a part of the Secure Knowledge Framework project\footnote{https://www.securityknowledgeframework.org/}. The OWASP\footnote{https://owasp.org/} Security Knowledge Framework (SKF) is a tool to guide developers to ensure security in all stages of software development. 

%SKF is available as an open source web application. SKF maintains a huge knowledge base of information related to different software security vulnerabilities. In addition to this, it tries to achieve secure development by providing security checklists for software projects. These checklists are derived from OWASP Application Security Verification Standard (ASVS) and Mobile Application Security Verification Standard (MASVS)\cite{cite6}. 


% \subsection{\textbf{SKF Chatbot}}
%SKF chatbot was developed by Jain et al. as an extension of the SKF project to enable the users to quickly access the required information on security vulnerabilities from the knowledge bases managed by SKF. Users can ask questions about various software vulnerabilities in natural language to the bot. The chatbot mainly attempts to answer 3 types of questions about these vulnerabilities: i) Description: The chatbot gives a detailed description in natural language for the given vulnerability ii) Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability iii) Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby.

%\begin{itemize}
%    \item Description: The chatbot gives a detailed description in natural language for the given vulnerability.
%    \item Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability.
%    \item Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby. 
%\end{itemize}

%\paragraph{\textbf{SKF Knowledge Base}}
%The SKF knowledge base consists of information about thousands of software security vulnerabilities and their code examples. One of the main sources for the data in this knowledge base is the CWE (Common Weakness Enumeration) list. In addition to the vulnerabilities in this list, SKF maintains and updates their own list of vulnerabilities. The knowledge base data can be found in their Github repository\footnote{https://github.com/blabla1337/skf-flask/tree/main/skf/markdown/knowled- ge\_base}.

SKF chatbot executes three main steps when answering users' queries: (i) intent classification, (ii) entity recognition, and (iii) response generation. In the first step, SKF seeks to understand whether the goal of the user is to get a description, a solution, or a code snippet. For this, it uses a Multinomial Naive Bayes (MNB) classifier to predict the question's intent. Next, it tries to identify the vulnerability for which the user is requesting information. This is done through a keyword-extraction algorithm named Rapid Automatic Keyword Extraction (RAKE), which is domain-independent and helps separating keywords from other words in the question. Finally, SKF generates a response by querying its knowledge base with the intent and the entities extracted from the user's question. \autoref{fig:chatbot} illustrates the output generated for \textit{``What is XSS?''}.

%The working of SKF chatbot can be divided into 3 main steps: \textit{i) Intent Classification}: First step in answering a natural language question from a user is to identify the intent behind the question. SKF chatbot uses a prominent Natural Language Processing (NLP) algorithm called Multinomial Naive Bayes (MNB) classifier to predict the intent of a question. 
%MNB classifier is a frequently employed algorithm to classify textual  data. 
%Based on the predictions from this probabilistic learning algorithm, the chatbot decides if the user is asking for the description, solution or a code example for the vulnerability. \textit{ii) Entity Recognition}: In this step, the chatbot tries to understand the vulnerability for which the user is requesting information. This is done by separating the keywords from the common words in the question. SKF chatbot achieves this with the help of a domain independent keyword extraction algorithm called Rapid Automatic Keyword Extraction (RAKE) \cite{cite10}. \textit{iii) Response Generation}: Depending on the intent and the entity extracted from the question, the bot generates a response by parsing the knowledge base.

%\paragraph{\textbf{SKF Chatbot Deployment}}
%SKF allows 2 ways to deploy and use the chatbot: Gitter\footnote{https://gitter.im/} and Terminal. Gitter is an open source instant messaging platform for software developers and Github users. The Gitter version of the chatbot allows users to chat with the bot in a chat room on Gitter platform. Alternatively, the terminal version allows the users to run the chatbot on their local machines via terminal. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[width=\linewidth]{figures/skf_short.jpeg}
    \caption{Terminal version of SKF chatbot}
    \label{fig:chatbot}
\end{figure}

%The terminal version of the chatbot was used in our study. A depiction of the chatbot answering questions in the terminal version is shown in Figure \ref{fig:chatbot}. 



==> SKF chatbot study/sections/result.tex <==
\section{Results} \label{sec:results}

We recruited 15 participants for our experiment (Groups A, B, and C of 4 participants each, and Group D with 3), most of them master students at \textit{*Anonymized Institution*}. In a preliminary assessment, participants' reported having low to medium knowledge on software security, while their general programming skills averaged in medium to high range which made them suitable candidates for evaluating the performance of SKF chatbot. In the following subsections we report our findings in terms of \textit{Effectiveness}, \textit{Q\&A Coverage}, and \textit{Perceived Usefulness}.

\subsection{Effectiveness}

To determine the DevBot's effectiveness, we analysed the number of vulnerabilities successfully fixed by the participants. We considered a vulnerability as ``fixed'' when the correct patch is applied along with the necessary libraries for executing it. When such libraries are not included, the vulnerability is considered as ``partially fixed''. A vulnerability is ``not fixed'' either when no patch is applied or when the wrong solution is implemented. 

Based on this criterion, we observed that for both vulnerabilities (i.e., XSS and SQLI) the number of full fixes was higher when no DevBot support was provided (\autoref{fig:effectiveness}). Particularly, 7 out of 15 participants managed to fully solve the given task by conducting an Internet search, but only 3 arrived to the right fix when receiving DevBot support. %This number was 4 against 2 full fixes when solving the SQLI vulnerability task.

When it comes to partial fixes, our results are mixed. As shown in \autoref{fig:effectiveness}-left, there were more participants arriving to a partial solution of the XSS vulnerability with the help of SKF chatbot (4) than using Internet search (1). Conversely, more participants arrived to a partial fix of the SQLI vulnerability without any DevBot support. Particularly, 2 participants arrived to a partial fix with the help of SKF chatbot, whereas 3 did it only by the means of Internet searches (\autoref{fig:effectiveness}-right). The number of unfixed vulnerabilities was for both tasks lower or equal when participants applied a self-conducted Internet search than a DevBot-assisted one.

%To assess SKF's efficiency we compared the time taken by the participants to finish the tasks with and without its support. Overall, the average time taken to complete one task (either XSS or SQLI) with SKF's assistance is 28.5 minutes, whereas when conducting an Internet search it is about 25.6 minutes.


\begin{comment}

\begin{table}[htbp]
\caption{Performance of the participants in removing the vulnerabilities}
\begin{center}
\begin{tabular}{|m{1cm}|c|c|c|c|}
\hline
\textbf{Status}&\multicolumn{2}{|c|}{\textbf{Without using SKF (\%)}} & \multicolumn{2}{|c|}{\textbf{Using SKF (\%)}}  \\
\cline{2-5} 
\textbf{} & \textbf{\textit{XSS}}& \textbf{\textit{SQLI}} & \textbf{\textit{XSS}}& \textbf{\textit{SQLI}} \\
\hline
Unsolved &   42.8 & 14.2 & 42.8 & 33.3 \\
Partially solved & 14.2 & 28.57 & 42.8 & 33.3 \\
Solved & 42.8 & 57.14 & 14.2 & 33.3 \\
\hline

\end{tabular}
\label{tab:performance}
\end{center}
\end{table}


\begin{figure}
    \centering
    \begin{tikzpicture}
\begin{axis}
    [
        ybar, 
        enlargelimits=0.4,
        legend style= {at = { (0.75,-0.15) }, legend columns = 1},
        ylabel = {Participants Percentage},
        symbolic x coords = {Unsolved, Partially solved, Solved},
        xtick = data,
        nodes near coords,
        nodes near coords align = {vertical},
        bar width = 20pt,
        fill
    ]
    \addplot coordinates {(Unsolved, 42.8) (Partially solved, 42.8) (Solved, 14.2) };
    \addplot coordinates {(Unsolved, 42.8) (Partially solved, 14.2) (Solved, 42.8) };
    \legend {Using SKF, Without Using SKF}

\end{axis}

\end{tikzpicture}
    \caption{Graph showing the performance of participants in fixing XSS vulnerability with and without using SKF chatbot }
    \label{fig:xssgraph}
\end{figure}

\end{comment}

\begin{figure*}[hbt!]
    \centering
    \includegraphics[width=0.40\linewidth]{figures/xss.jpeg}\hspace{2ex}
    \includegraphics[width=0.40\linewidth]{figures/sqli.jpeg}
    \caption{Participant's performance when fixing the XSS (left) and the SQLI vulnerabilities (right).}
    \label{fig:effectiveness}
\end{figure*}

\begin{comment}

\begin{figure}
    \centering
    \begin{tikzpicture}
\begin{axis}
    [
        ybar, 
        enlargelimits=0.4,
        legend style= {at = { (0.75,-0.15) }, legend columns = 1},
        ylabel = {Participants Percentage},
        symbolic x coords = {Unsolved, Partially solved, Solved},
        xtick = data,
        nodes near coords,
        nodes near coords align = {vertical},
        bar width = 20pt,
        fill
    ]
    \addplot coordinates {(Unsolved, 33.33) (Partially solved, 33.33) (Solved, 33.33) };
    \addplot coordinates {(Unsolved, 14.20) (Partially solved, 28.57) (Solved, 57.14) };
    \legend {Using SKF, Without Using SKF}

\end{axis}

\end{tikzpicture}
    \caption{Graph showing the performance of participants in fixing SQL injection vulnerability with and without using SKF chatbot }
    \label{fig:sqlgraph}
\end{figure}


\end{comment}

\subsection{Q\&A Coverage} \label{sec:qacoverage}

Another aspect relevant to the DevBot's performance is the amount of questions it manages to answer. Hence, we asked participants whether SKF chatbot responded to all of their questions to understand to which extent it helped in the resolution of the tasks. All in all, 10 out of 15 participants mentioned that SKF chatbot answered all of their questions, while 3 said it only answered them partially. The remaining 2 participants reported not receiving any useful information from the DevBot for addressing the security vulnerabilities.

To further assess SKF's Q\&A coverage, we asked participants whether they used other resources (e.g., Internet search) in addition to the DevBot for fixing the vulnerabilities. From 15 participants, 9 reported having used additional resources to complete the given task, whereas 6 mentioned that they did not. Among the 9 participants who used extra resources, 5 of them had reported that the DevBot did answer all of their questions. 



\subsection{Perceived Usefulness}\label{sec:usefulness}

There are two main steps when removing a vulnerability from a software application, namely (i) understanding the nature of the vulnerability, and (ii) finding the correct fix for such a vulnerability. In order to analyse how well SKF chatbot supports this process, we asked participants whether they would prefer a DevBot over an Internet search on each of these stages or not. 

As shown in Figure \ref{fig:preferences-graph}, 12 out of 15 participants reported that using SKF chatbot helped them to better understand the vulnerability than simply searching for it on the Internet. On the other hand, opinions were more polarized when it comes to finding the right fix. Particularly, 7 out of 15 respondents said they rather look for the correct fix themselves using the Internet, while 8 opted for a DevBot-supported search. Interestingly, only 3 out of 15 participants managed to find full fixes (i.e., either XSS or SQLI) with the help of SKF chatbot. However, if we consider the the total number of full and partial fixes with DevBot support we obtain 9 out of 15, which is closer to the fixing preferences reported by the participants.

%Overall, this last number approaches 9, which is the total full and partial fixes with DevBot intervention (5 from the XSS task and 4 from the SQLI task). 
%This is particularly interesting because, out of the 15 participants only 3 of them were able to completely remove a vulnerability (i.e., either XSS or SQLI) with the help of SKF chatbot, while 7 successfully managed to remove the vulnerability without such a help.

\begin{figure}[hbt!]
    \centering    \includegraphics[width=0.95\linewidth]{figures/understood_removed_new.jpeg}
    \caption{Participants' preferences regarding understanding and removing security vulnerabilities.}
    \label{fig:preferences-graph}
\end{figure}

%This was expected because the 80\% of the participants voted yes or partially yes when they were asked if the bot answered all their  questions. 


Last but not least, we asked a subgroup of participants (8) if they would use a conversational DevBot for addressing security vulnerabilities in the future. The available options were \textit{yes}, \textit{no} and \textit{maybe}. Overall, there was only one participant who was willing to receive DevBot support for applying future security fixes, whereas 5 said they might and 2 that they wont.

%\subsection{Overall Acceptance}

%To shed more light into the preferences of the participants, we asked them which method they would prefer to deal with software security vulnerabilities as a whole and the reasoning behind it. 6 participants identified SKF chatbot as a potential tool that can help in removing vulnerabilities in an application. 

%Out of the participants who did not choose using SKF chatbot as the preferred method to remove security vulnerabilities, 4 of them picked browsing the internet as the preferred method and the remaining 5 did not give any preferences. A major factor which was identified by multiple participants as a limiting component of the chatbot is its lack of versatility. 

%Few participants also pointed out that the way the answers are presented by the chatbot is very primitive making it difficult to read and understand. We asked the participants of the second phase of the experiment, if they would use SKF chatbot in the future to deal with software security vulnerabilities. Even though multiple participants of the second phase of the experiment stated that using SKF chatbot helps better to remove vulnerabilities, only one of them voted yes to use SKF chatbot in the future. The remaining participants appear to be less confident in the chatbot to assist in software security related matters.


==> SKF chatbot study/sections/study.tex <==
\section{\textbf{Research Methodology}}
\label{sec:methodology}

Despite being one of the few (for not saying the only) security DevBots with conversational features, SKF's usability has not been yet thoroughly investigated to the best of our knowledge. Hence, we conducted and empirical study to analyse its performance, efficiency, and overall user acceptance. In the following subsections we describe the proposed experimental setting along with the instruments used for SKF's assessment.


%The goal of this study is to understand the extent to which a conversational security DevBot can assist software developers in writing secure code. To the best of our knowledge, SKF chatbot is one among the very few  conversational security DevBots which are available as an open source project. Hence we used SKF chatbot to conduct this study. A detailed description of the steps we followed to conduct this study are given in the following subsections.


\subsection{\textbf{Experimental Setup}}

We conducted the evaluation of SKF chatbot using a Java web application containing 2 code-level security vulnerabilities allowing Cross-Site Scripting (XSS) and SQL Injection (SQLI) attacks. While the former consists of placing of malicious SQL code inside webpage inputs, the latter occurs when malicious code is sent through a web application (usually as browser-side scripts). The participants were given the source code of this web application in which the locations of the vulnerabilities were marked in comments. They were asked to fix the specified vulnerable area of the code with and without SKF's help. For this, we created 4 groups, each receiving the tasks and the DevBot support in a different order to reduce the presence of biases in our analysis (\autoref{fig:workflow}). For instance, participants in \textit{Group A} had to fix the XSS vulnerability first and then the one corresponding to SQLI. In this case, the support of SKF chatbot was given for the resolution of the second task (i.e., SQLI), whereas for the first one (i.e., XSS) they were only allowed to use Internet search.

 %As a part of this experiment, we developed a  Java web application that contains 2 code-level security vulnerabilities. The participants of this experiment were asked to remove these vulnerabilities with and without the help of SKF chatbot. After each task, the participants filled out survey forms for us to record the influence of the presence and absence of the chatbot in performing the task. An overview of our empirical study setup is shown in Figure \ref{fig:workflow}. To avoid biases caused by the order in which the tasks are performed, the participants were divided into 4 groups. Participants in Groups A and C had to remove cross-site scripting (XSS) vulnerability in the first task and SQL injection in the second task whereas Groups B and D had to do the tasks in the reverse order. Additionally, groups A and B performed the first task without using SKF chatbot and  the second task using SKF chatbot. On the other hand, groups C and D used SKF chatbot in the first task and performed the second task without the chatbot. Thus, the 4 groups performed the tasks in different orders to reduce the possibility of biases in the results.  
 
\begin{comment}

The task distribution for each of these 4 groups are shown in Table \ref{table:task}. 
 
 \begin{table}[hbtp]
\centering
\caption{\label{table:task} Task Distribution}
\begin{tabular}{ |c|c|c| } 
\hline
     \textbf{Group} & \textbf{Task 1} & \textbf{Task 2} \\ 
 \hline
     A & XSS  (Without Bot) & SQLI  (With Bot) \\ 
     B & SQLI  (Without Bot) & XSS  (With Bot) \\ 
     C & XSS  (With Bot) & SQLI  (Without Bot) \\ 
     D & SQLI  (With Bot) & XSS  (Without Bot) \\ 
 \hline
 
\end{tabular}

\end{table}
 
 
\end{comment}
 
 
 
 \begin{figure}[hbt!]
    \centering
    \includegraphics[width=\linewidth]{figures/study.png}
    \caption{Workflow of the empirical study}
    \label{fig:workflow}
\end{figure}

\begin{comment}
\subsection{\textbf{Vulnerable Web Application}}
The vulnerable web application used in this study is a simple login page. Java being a popular language and one of the languages supported by the SKF chatbot, we chose Java to develop this web application. The web application contains  2 software security vulnerabilities that enables 2 kinds of security attacks : SQL Injection (SQLI) \cite{cite12} and Cross Site Scripting (XSS) \cite{cite13}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=.13]{figures/webapp1.jpeg}
    \caption{Welcome page of the vulnerable web application}
    \label{fig:webapp}
\end{figure}


\subsubsection{SQL Injection}
 SQL Injection (SQLI) is an attack technique where the attackers try to gain access to the backend database by inserting malicious SQL code into the application's input fields. 
 %Our vulnerable web application maintains a database of users. This database stores the username and the password of the users. 
 The application verifies the entered username and password in the login page by querying a backend database. 
 %If there is a match, the application displays 'Login Successful' and if there is no match, the application displays 'Login Failed' on the web page. 
 The SQL query used to verify the username and password is as follows: 
 
 \texttt{SELECT * FROM tbluser WHERE} 
 
 \texttt{username='" + username + "' AND} 
 
 \texttt{password = '" + password + "'"}
 
 Here, \texttt{tbluser} is the table in the database in which the usernames and the passwords are stored. This query is susceptible to SQL injection attack. If the attacker enters the value \texttt{'or '1'='1} into the username or password field in the application, the condition check in the above SQL query will be bypassed enabling the attacker to login without the correct username or password. 

\subsubsection{Cross-Site Scripting}
Cross-site scripting (XSS) is a vulnerability found in web applications that allows attackers to inject malicious code into a web page viewed by other users. 

In our web application, there is a greetings section where the users can enter their name.  When the Submit button is pressed, the application displays a message \textit{'Hello $\langle name \rangle$'}.  The HTML script that performs this action in the application is shown below:
\begin{verbatim}
<html>
  <body>
   <h1 align='center'> Hello $name </h1>
  </body>
</html>
\end{verbatim} 

In the above code snippet, the variable \texttt{\$name} holds the string entered by the users in the application. An attacker could use this input field to insert scripts that perform unwanted actions. An example attack script is given below:

\begin{verbatim}
<iframe src="javascript:alert(`Hacked!`)">
\end{verbatim}

The above script, when entered into the input field will display a pop-up message that says \textit{'Hacked!'} on the web application. 

\end{comment}


\subsection{\textbf{Survey Instruments}}

We created 3 survey forms for the experiment containing yes/no, multiple choice, and open-ended questions. Survey  1 was given to the participants after completing the first assignment, whereas Survey 2 and 3 after the second task. Particularly, Surveys 1 and 2 were tailored according to (i) the task the participant had to solve, and (ii) whether she received support of SKF chatbot for its resolution or not. For instance, participants in Group A were asked about the use of online sources for fixing the XSS vulnerability in Survey 1, while in Survey 2 they provided feedback on the use of the conversational DevBot (e.g., their perceived usefulness). Survey 3 remained the same for every group and was given to the participants at the very end of the experiment. Particularly, it contained questions eliciting participants' overall acceptance of the DevBot when solving security vulnerabilities (e.g., if they preferred the DevBot's assistance over a self-conducted Internet search). This third form also included open-ended questions aiming to collect user input that could help shaping additional features for the DevBot. All survey forms and task descriptions were compiled into a \textbf{supplementary~file} available inside a public repository\footnote{Repository link: \url{https://collaborating.tuhh.de/e-22/public/skf-chatbot-empirical-study}.}.

%available inside a GitLab repository \footnote{https://collaborating.tuhh.de/e-22/public/skf-chatbot-empirical-study}.

%We used a total of 3 surveys to collect relevant information from the participants of the experiment. Every survey included yes or no, multiple choice and long answer questions. The questions of the survey forms were designed to help us answer the previously mentioned 4 research questions. The structure of each of these surveys are explained below.

 
 %\subsubsection{Survey for the task without using SKF chatbot}
 %After finishing the task that \textbf{does not involve the usage of SKF chatbot}, the participants were given a survey. Questions in this survey were designed to understand how well online sources of programming information like  Google, Github, Stack Overflow etc. helped in understanding and removing the security vulnerability in the application. 
 
 %A few questions from this survey are given below:
 
 %\begin{itemize}
 
%     \item Do you fully understand what the vulnerability is and how it is exploited?
%     \item If you googled to resolve the vulnerability, what information did you search for?
%     \item Were you able to remove the security vulnerability by using a web search engine (eg. Google) or with your prior knowledge? 
%     \item Briefly explain the vulnerability and the fix for the vulnerability in your own words.
     
% \end{itemize}
 
 %\subsubsection{Survey for the task using SKF chatbot}
 %This survey was given at the end of the task which involves the usage of SKF chatbot. It contains questions specifically related to SKF chatbot to  evaluate the SKF chatbot in terms of its knowledge coverage, understandability and effectiveness in assisting the participant to remove vulnerability from the code. We also collect the participant's feedback on SKF chatbot as a whole in this survey form. 
 
 %A few questions from this survey are given below:
 
 %\begin{itemize}
 
 %    \item Were you able to solve the security vulnerability by using SKF Chatbot? 
 %    \item Did SKF Chatbot respond with answers to all your questions regarding security issues? 
 %    \item Do you fully understand what the vulnerability is and how it is exploited?
 %    \item How would you rate the usefulness of the SKF chatbot?
    
     
 %\end{itemize}
 
 %\subsubsection{Survey for comparing the 2 approaches}
 %This is the final survey which is given to the participants after finishing the second survey at the end of the second task of the experiment. The purpose of this survey is to compare the two approaches used in this experiment (with chatbot and without chatbot) by collecting the preferences of the participants. 
 
 %The above mentioned survey forms can be found in our Git repository\footnote{https://collaborating.tuhh.de/e-22/catherine-tony/skf-chatbot-study}.
 
 %A few questions from this survey are given below.
 
 %\begin{itemize}
 %    \item Which of the below cases is more useful to help you understand a vulnerability? 
 %    \item Which of the below cases is more useful to help you remove a vulnerability? 
 %    \item Which of the two methods would you prefer and why? 
 %\end{itemize}
 
 
 %%Below is the list of questions which we used to answer our initial 3 research questions.

%%\textbf{\textit{RQ1:} How useful are conversational DevBots in secure programming?}
%%\begin{itemize}
%    \item Were you able to remove the vulnerabilities by using SKF chatbot?
   
%    \item Did the chatbot respond with satisfying answers to all the questions? If not, which are the questions that were unanswered?
%    \item Did you feel the need to use any other resources in addition to the chatbot to finish the task?
%    \item Which of the following was more useful for you to understand the vulnerabilities?
%    \begin{itemize}
%        \item Using SKF chatbot
%        \item Using other resources
%    \end{itemize}
%    \item Which of the following was more useful for you to remove the vulnerabilities? 
%    \begin{itemize}
%        \item Using SKF chatbot
%        \item Using other resources
%    \end{itemize}
    
%%\end{itemize}

%%In addition to the above questions, we also analysed the Java source code submitted by the participants to compare the solutions obtained using both the methods.



%%\textbf{\textit{RQ2:} How efficient is the use of conversational DevBots in supporting the developers to remove security vulnerabilities from software applications?}
%%\begin{itemize}
%%    \item How much time did you take to solve the vulnerability?
%%    \item Did SKF Chatbot respond with answers to all your questions regarding security issues?
%%        \begin{itemize}
%%            \item If no, list the questions the chatbot failed to answer.
%        \end{itemize}
%%\end{itemize}


%%\textbf{\textit{RQ3:} Do developers prefer to use a conversational DevBot to assist with code security tasks?}
%%\begin{itemize}
%    \item Which one of the 2 methods do you prefer to solve security vulnerabilities and why?
       
%    \item Would you use SKF chatbot or any other chatbot in the future for secure programming?
    
%%\end{itemize}

%\textbf{\textit{RQ4:} What features do developers expect in a conversational DevBot for secure programming?}
%\begin{itemize}
%    \item What did you like about SKF chatbot?
%    \item What did you dislike about SKF chatbot?
%    \item What additional features would you like to have in the chatbot?
%\end{itemize}


\begin{comment}
\subsection{\textbf{Study Participants}}
The data collection for this study was carried out in 2 phases. The first phase was conducted with 7 participants in the month of September. The participants included master students as well as professionals in the field of computer science. The second phase consisted of 8 participants and was conducted in the month of December. The participants of the second phase were master students in a software security course. There were slight changes in the surveys filled by the participants of both the phases. But we believe that the changes in the forms are minimal enough to consider the participants of both the phases as one single group and analyse the data from both the groups together. Before the experiment, we collected some preliminary information from all the participants to capture their programming and software security background. 

Following are few of the information we collected from each of the participants to account for biases in the study results.

\begin{enumerate}
    \item Knowledge on Java programming language (The web application is written in Java)
    \item Knowledge in SQL (The backend database is queried using SQL)
    \item General programming knowledge
    \item Professional software development experience
    \item Knowledge in software security vulnerabilities
\end{enumerate}




\begin{table}[hbtp]
\centering
\caption{\label{table:participants} Overview of the study participants. 1 is the lowest level and 5 is the highest level.}
\begin{tabular}{ |m{0.5cm}|m{1.4cm}|m{1.4cm}|m{1.6cm}|m{1.7cm}| } 
\hline
     \textbf{Level} & \textbf{Java Knowledge} & \textbf{SQL Knowledge} & \textbf{General Programming Knowledge} & \textbf{Software Vulnerabilities Knowledge} \\ 
 \hline
 
     1 & 0\%  & 13.33\% & 0\% & 13.33\%\\ 
     2 & 53.33\%  & 60\% & 6.66\% & 53.33\%\\ 
     3 & 33.33\%  & 13.33\% & 40\% & 26.66\%\\ 
     4 & 13.33\%  & 13.33\% & 53.33\% & 6.66\%\\ 
     5 & 0\%  & 0\% & 0\% & 0\%\\ 
 \hline
 
\end{tabular}

\end{table}

 An overview of some of the information collected about the participants are shown in Table \ref{table:participants}. The first column indicates the level of knowledge or expertise one has in a given topic. Level 1 indicates very poor knowledge while level 5 indicates very good knowledge. The values in the remaining columns give the percentage of the total participant belonging to a particular level of expertise for the given topic. Only 46.66\% and 26.66\% of the participants have average or above average knowledge in Java and SQL respectively while 93.33\% of the participants have decent knowledge of programming in general. From the table it is evident that no one among the participants have very good knowledge on software vulnerabilities. Majority percentage of the participants have very poor to somewhat average knowledge in the security vulnerabilities. This is exactly the kind of software developer population which is targeted by tools like SKF chatbot. In addition to the information shown in the table, out of the 15 participants, 7 of them have professional software development experience of approximately 1.5 years. From these information, we believe that our study participants make a fitting  group for this empirical study.
\end{comment}

==> sections/approach.tex <==
\section{\textbf{Background: SKF Chatbot}}
\label{sec:approach}

SKF chatbot \cite{cite5} was selected to study the relevance and effectiveness of conversational DevBots in secure software development. SKF chatbot is developed as a part of the Secure Knowledge Framework project\footnote{https://www.securityknowledgeframework.org/}. 
%\subsection{\textbf{Security Knowledge framework (SKF)}}
The OWASP\footnote{https://owasp.org/} Security Knowledge Framework (SKF) is a tool to guide developers to ensure security in all stages of software development. It uses OWASP Application Security Verification Standard\cite{cite7} to educate programmers about software security vulnerabilities and how to prevent them. 

%SKF is available as an open source web application. SKF maintains a huge knowledge base of information related to different software security vulnerabilities. In addition to this, it tries to achieve secure development by providing security checklists for software projects. These checklists are derived from OWASP Application Security Verification Standard (ASVS) and Mobile Application Security Verification Standard (MASVS)\cite{cite6}. 


% \subsection{\textbf{SKF Chatbot}}
SKF chatbot was developed by Jain et al. \footnote{https://github.com/Priya997/SKF-Chatbot} as an extension of the SKF project to enable the users to quickly access the required information on security vulnerabilities from the knowledge bases managed by SKF. Users can ask questions about various software vulnerabilities in natural language to the bot. The chatbot mainly attempts to answer 3 types of questions about these vulnerabilities: i) Description: The chatbot gives a detailed description in natural language for the given vulnerability ii) Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability iii) Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby.

%\begin{itemize}
%    \item Description: The chatbot gives a detailed description in natural language for the given vulnerability.
%    \item Solution: The chatbot gives a detailed explanation of the approach to solve the vulnerability.
%    \item Code Snippet: The chatbot gives examples of code for the solution in a specified language. Currently the bot supports Django, Java, PHP, Flask and Ruby. 
%\end{itemize}

\paragraph{\textbf{SKF Knowledge Base}}
The SKF knowledge base consists of information about thousands of software security vulnerabilities and their code examples. One of the main sources for the data in this knowledge base is the CWE (Common Weakness Enumeration) \cite{cite11} list. In addition to the vulnerabilities in this list, SKF maintains and updates their own list of vulnerabilities. The knowledge base data can be found in their Github repository\footnote{https://github.com/blabla1337/skf-flask/tree/main/skf/markdown/knowled- ge\_base}.
\paragraph{\textbf{Working of SKF Chatbot}}

The working of SKF chatbot can be divided into 3 main steps: \textit{Intent Classification, Entity Recognition and Response Generation}

Intent Classification: First step in answering a natural language question from a user is to identify the intent behind the question. SKF chatbot uses a prominent Natural Language Processing (NLP) algorithm called Multinomial Naive Bayes (MNB) classifier to predict the intent of a question. MNB classifier is a frequently employed algorithm to classify textual data. Based on the predictions from this probabilistic learning algorithm, the chatbot decides if the user is asking for the description, solution or a code example for the vulnerability.

Entity Recognition: In this step, the chatbot tries to understand the vulnerability for which the user is requesting information. This is done by separating the keywords from the common words in the question. SKF chatbot achieves this with the help of a domain independent keyword extraction algorithm called Rapid Automatic Keyword Extraction (RAKE) \cite{cite10}.

Response Generation: Depending on the intent and the entity extracted from the question, the bot generates a response by parsing the knowledge base.

\paragraph{\textbf{SKF Chatbot Deployment}}
SKF allows 2 ways to deploy and use the chatbot: Gitter\footnote{https://gitter.im/} and Terminal. Gitter is an open source instant messaging platform for software developers and Github users. The Gitter version of the chatbot allows users to chat with the bot in a chat room on Gitter platform. Alternatively, the terminal version allows the users to run the chatbot on their local machines via terminal. The terminal version of the chatbot was used in our study. A depiction of the chatbot answering questions in the terminal version is shown in Figure \ref{fig:chatbot}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=.2]{figures/skf.jpeg}
    \caption{Terminal version of SKF chatbot}
    \label{fig:chatbot}
\end{figure}

==> sections/extras.tex <==

%--DONE: One of the main reasons is the ease with which one can retrieve information from the chatbot. A serious problem developers face while browsing the internet for answers is the overwhelming amount of information. The enormous number of sources on the internet makes it sometimes difficult to retrieve the relevant information. SKF chatbot helps in significantly reducing the information retrieval time and effort. SKF chatbot provides the description of the vulnerability, explains the mitigation methods and gives code examples for the defense methods which makes it extremely convenient for the developers to use it. The chatbot also allows the users to choose the programming language for the code example they request. Another advantage of SKF chatbot identified by few participants is its reliability. Even though you can find a large amount of information on the internet, it is often hard to decide the reliability and correctness of these information. SKF chatbot is specially designed to address software security related issues. Hence it can be considered as a more trusted source of information for software security. One participant pointed out the clarity and understandability of the answers given by the chatbot as a contributing factor in choosing the SKF chatbot for the removal of vulnerabilities. Some participants also appreciated the interactive nature of the chatbot. 

%--DONE: Despite getting satisfactory answers from the bot, many of the participants were not able to solve the task using SKF chatbot while using other information resources proved to give better results. After further inspection of the unanswered questions from the participants who did not get completely satisfactory answers, we found some  limitations of the bot. One of the major drawbacks identified by the participants was that the bot only responds to specific questions. 

%--DONE: The three main responses one can obtain from SKF chatbot are the description of the vulnerability, mitigation methods and code example for these mitigation methods. It is natural for the users to have follow up questions after looking at the answers given by the bot. However, the chatbot grants no provision to ask such questions. More accurately, there are indeed provisions to ask follow up questions, but the chatbot merely responds with either the same answers or fails to answer all together. Another participant mentioned that the chatbot did not have information on the external libraries used to implement a solution.  One participant pointed out the lack of domain knowledge of the chatbot. The information provided by the chatbot on the vulnerabilities were found insufficient to fully comprehend and fix the vulnerabilities.

%--DONE: To clarify the disparity in this data, a follow up interview was conducted with the 5 participants to explain their decisions. Few of the responses are given below.

%--DONE: \begin{quote}
%    \textit{P4: For someone who was a beginner at such tasks, I needed more examples with explanation. But it was a good point to start. From the points given by the chatbot I understood what exactly I need to search. }
%\end{quote}

%--DONE: \begin{quote}
%    \textit{P9: I was looking into other resources to look for specific Java code examples, i.e. API calls. So for me, it was accompanying material, as the chatbot helped me to nail down the problem itself and give me “trustworthy” information.}
%\end{quote}

%--DONE: From the above responses, we observed that the contrasting feedbacks are caused by how different participants perceive the chatbot. While some of them see the chatbot as a starting point for their search for answers, the others see it as the sole source of information to perform a task.

%\subsection{Overall Acceptance}

%Quotes from a few participants are given below regarding the versatility of the chatbot.

%---DONE:\begin{quote}
%    \textit{P9: " My question had to match the given question exactly. I ended up with asking for very broad topics and then selecting from the given list of options to find exactly what I was looking for. "}
%\end{quote}
%\begin{quote}
%    \textit{P12: " to me the bot was not really useful, because i asked different questions and got always the same answer, .. "  }
%\end{quote}

%--DONE: If the participants are choosing to not use a conversational agent that is specially designed to make their life easier then definitely the agent is missing some important features. To understand this we asked the participants about the features and characteristics they expect in such a conversational agent. Some participants mentioned that they would prefer to have a better user interface for a chatbot. The messages from the chatbot especially those that involve a large amount of text should be well formatted to make it more readable. One additional feature suggested by few of the participants is an indication of the security level of the solutions. 

%--DONE: Security vulnerabilities in software applications can be solved in multiple ways. Developers often find it hard to decide which solution to implement for their use case. It would be helpful if the chatbot can indicate how secure a given solution is. 

%--DONE: Most participants expect chatbots to have much more domain knowledge instead of limiting the questions just to description, mitigation and code examples. Expanding the code examples to more programming languages will also be a good addition to the chatbot. A few participants found it difficult to integrate the code examples for the solutions given by the chatbot into their own project. They pointed out that it would be very useful if the chatbot provided assistance in doing this. 
